An optimal-transport finite-particle method for mass diffusion

We formulate a class of velocity-free finite-particle methods for mass transport problems based on a time-discrete incremental variational principle that combines entropy and the cost of particle transport, as measured by the Wasserstein metric. The incremental functional is further spatially discretized into finite particles, i.e., particles characterized by a fixed spatial profile of finite width, each carrying a fixed amount of mass. The motion of the particles is then governed by a competition between the cost of transport, that aims to keep the particles fixed, and entropy maximization, that aims to spread the particles so as to increase the entropy of the system. We show how the optimal width of the particles can be determined variationally by minimization of the governing incremental functional. Using this variational principle, we derive optimal scaling relations between the width of the particles, their number and the size of the domain. We also address matters of implementation including the acceleration of the computation of diffusive forces by exploiting the Gaussian decay of the particle profiles and by instituting fast nearest-neighbor searches. We demonstrate the robustness and versatility of the finite-particle method by means of a test problem concerned with the injection of mass into a sphere. There test results demonstrate the meshless character of the method in any spatial dimension, its ability to redistribute mass particles and follow their evolution in time, its ability to satisfy flux boundary conditions for general domains based solely on a distance function, and its robust convergence characteristics.

==> Beta.tex <==

We implemented the optimization of the parameter $\beta_p$ for each particle $p$, according to Eq.~\eqref{Xn0flD}. However, $\beta_p$ values are lower- and upper-bounded by restrictions related to boundary conditions and by numerical considerations. A lower-bound is imposed by the domain size $D$, giving $\beta_{\rm min} = 1/D^2$, as too small values of $\beta_p$ (i.~e., a large interaction neighborhood for the particle) will assign to all particles the same effect independently of the relative distance from the particle $p$. An upper-bound is associated with the mesh size, giving $\beta_{\rm max} = 1/dx^2$, as too large values of $\beta$ (i.~e., a small interaction neighborhood) will isolate the particle, making it unable to perceive the presence of the surrounding particles. 

Because of the presence of $n$ in the left-hand-side of Eq.~\eqref{Xn0flD}, for large $n$ values, the optimized $\beta_p$ kicks always the upper-bound. It follows that, if a good initial value of $\beta_p = \bar \beta$ is assigned to all the particles, the $\beta_p$ optimization becomes redundant, and it is shut down to save computational time.

The distance $dx$, Eq.~\eqref{eq:meshSize}, can be used to estimate the ``optimal average'' $\bar \beta$. Since $\beta$ has the dimensions of the inverse of a squared length, we have considered the following three relations that link the number of particles $n$ to $\bar \beta$ as a power law
\begin{equation}
    \label{eq:betaEstimate}
    \bar \beta_1 \approx \frac{1}{dx^2} = C_1 \frac{n^{2/3}}{R^2} \, ,
\end{equation}
which corresponds to the upper-bound $\beta_{\rm max}$;
\begin{equation}
    \label{eq:betaEstimate2}
    \bar \beta_2 \approx \frac{1}{dx R} = C_2 \frac{n^{1/3}}{R^2} \, ,
\end{equation}
which is a weighed measure between the domain size $D$ and the mesh size $dx$; and
\begin{equation}
    \label{eq:betaEstimate3}
    \bar \beta_3 = \sqrt{\bar \beta_1 \bar \beta_2} \approx
    \sqrt{\frac{1}{dx^3 R}} = C_3 \frac{n^{1/2}}{R^2} \, ,
\end{equation}
which is an average between the previous two measures. Fig.~\ref{Fig:BetaParticles} visualizes the dependence of the average $\bar \beta$ parameters on the number of particles $n$.
\begin{figure}
    \centering
    \includegraphics[width = 0.75\textwidth]{betaParticles.jpg}
    \caption{\footnotesize Example of the injected sphere. Dependence of the average $\bar \beta$ parameter, according to the expressions given in Eqs.~\eqref{eq:betaEstimate}-\eqref{eq:betaEstimate3}, on the number of particles. The plot shows also the dependence of the minimum distance $dx$ on the number of particles.}
    \label{Fig:BetaParticles}
\end{figure}
The constants $C_1$, $C_2$ and $C_3$ must be calibrated numerically. For the example shown in Section~\ref{sec:NumericalExperiments}, the best performance over a wide range of $n$ was offered by the expression \eqref{eq:betaEstimate3} with $C_3=10$, which has been used in all the calculations.


==> Convergence.tex <==

\section{Convergence analysis (old)}
\label{sec:Convergence}
The convergence of the method is evaluated by introducing an error function $E$, defined as 
\begin{equation}\label{eq:cost}
    E 
    =
    \int_0^T \sum_{p=1}^N {|v_p|^2 m_p} dt
    \approx \sum_{k=1}^{N_{\rm steps}} {\sum_{p=1}^N {|v_p|^2 m_p}} \Delta t_N \, ,
\end{equation}
where $T$ is the time for the diffusion process to take place, $v_p$ the velocity of the particle, and $N_{\rm steps}$ the number of time integration steps. 
We notice that, assigned the number of particles $N$, there is a direct relationship between $N$ and $\Delta t_N$.
The average distance between the particles can be evaluated as follows. If $R$ is the spherical container radius, the volume occupied by each particle can be estimated as the ratio between the volume of the container and $N$:
\begin{equation}\label{eq:distance}
    \frac{4}{3} \pi dx^3  
    =
     \frac{4}{3} \pi R^3 \frac{1}{N} \, .
\end{equation}
The stable time step $\Delta t_N$ is obtained by the Courant equivalent condition
\begin{equation}\label{eq:criticalTime}
    \Delta t_N  
    =
    \frac{dx^2}{\kappa} \, .
\end{equation}
The relation between the number of particles and the stable time step is
\begin{equation}\label{eq:N_Time}
    \Delta t_N  
    =
    \frac{R^2} {\kappa } N^{-2/3} \, .
\end{equation}

{\red A comment, not to forget what I have done in the last three days. The expression \eqref{eq:searchLimit} is not correct from the dimensional point of view, since $\epsilon$ is a dimensionless tolerance, while $N$ is the inverse of a volume. Apparently, this is responsible of the alignment of the particles on lines and planes. By considering instead $\epsilon$ as a percentage of the maximum value of the shape function, i.~e.,
\begin{equation}\label{eq:searchLimit2}
    \epsilon =
    \exp\Big( -\beta_p \| x - x_p \|^2 \Big) \, ,
\end{equation}
we obtain as maximum search radius
\begin{equation}\label{eq:searchDistance2}
    r_{\rm max}^2 = - \frac{1}{\beta_p}\log {\epsilon} \, .
\end{equation}
}

We then compare the cost function for different cases. 

\begin{table}[!h]
    \centering
    \begin{tabular}{cccc}
         \hline
         $n$ & $Cost$ & CPU Time RK [s] & CPU Time E [s]  \\
         \hline
         100 & -80,176 & 7 & 2      \\
         200 & -68,659 & 17 & 3     \\
         400 & -43,675 & 38 & 9     \\
         800 & -7,376  & 435  & 49  \\
         1600 & -545   & -    & 173 \\
         3200 & +875   & -    &     \\
         6400 &        &      & 1,631
    \end{tabular}
    \caption{Cases considered in the numerical experiments.}
    \label{table:cases}
\end{table}


==> Estimate.tex <==

\begin{equation}
\begin{split}
    &
    M 
    \frac{d}{2}\frac{1}{\beta_{k+1}}
    = \\ &
    \sum_{p=1}^n
        \Big(
            \frac
            {
                \sum_{q=1}^n
                    \| x_{p,k+1} - x_{q,k+1} \|^2
                    \Big( \frac{\beta_{k+1}}{\pi} \Big)^{d/2}
                    \,{\rm e}^{- \beta_{k+1} \| x_{p,k+1} - x_{q,k+1} \|^2 }
                \, m_q 
            }
            {
                \rho_{k+1}(x_{p,k+1})
            }
        \Big)
    \, m_p ,
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    &
    M 
    \frac{d}{2}\frac{1}{\beta_{k+1}}
    = \\ &
    \sum_{p=1}^n
        \Big(
            \frac
            {
                \int_\Omega
                    \| x_{p,k+1} - y \|^2
                    \Big( \frac{\beta_{k+1}}{\pi} \Big)^{d/2}
                    \,{\rm e}^{- \beta_{k+1} \| x_{p,k+1} - y \|^2 }
                    \rho(y)
                \, dy
            }
            {
                \rho_{k+1}(x_{p,k+1})
            }
        \Big)
    \, m_p ,
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    &
    M 
    \frac{d}{2}\frac{1}{\beta_{k+1}}
    = \\ &
    \int_\Omega
        \int_\Omega
            \| x - y \|^2
            \Big( \frac{\beta_{k+1}}{\pi} \Big)^{d/2}
            \,{\rm e}^{- \beta_{k+1} \| x - y \|^2 }
            \rho(y)
        \, dy
    \, dx,
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    &
    N 
    \frac{d}{2}\frac{1}{\beta_{k+1}}
    = % \\ &
    \Big( \frac{\beta_{k+1}}{\pi} \Big)^{d/2}
    \frac{d}{2}\frac{1}{\beta_{k+1}}
    |\Omega|
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    &
    N 
    = % \\ &
    \Big( \frac{\beta_{k+1}}{\pi} \Big)^{d/2}
    |\Omega|
\end{split}
\end{equation}


==> Searches.tex <==

The rate-limiting step in this approach is the operation of searching for the local neighborhood lists as they evolve during a simulation as a result of the relative motion of the particles. Numerous techniques have been developed for solving the local-neighborhood problem. One approach makes  use of space partitioning algorithms where the branch and bound method \cite{Land:2010} is applied. Early examples in this class are the $k$-d tree \cite{Bentley:1975, Friedman:1977} and the $k$-means algorithms \cite{Fukunaga:1975}, with many variants thereof. A deficiency of exact methods is that they cannot guarantee logarithmic search time \cite{Uhlmann:1991, Sproull:1991}. Conveniently, for many applications approximate nearest-neighbor (ANN) algorithms, which trade-off accuracy for efficiency, suffice \cite{Muja:2009b}. The scalability of the algorithms is assessed in \cite{Muja:2014}. More recent work has focused on proximity graph-based methods \cite{Li:2019, Groh:2019}, which are well-suited to high-dimensionality problems arising e.~g., in image recognition, computational linguistics, product recommendation, and others. 

The best choice of search algorithm depends on data-related properties such as dimension, data-set size, correlations, density distribution, and others, and performance metrics such as query time, accuracy, query workload, building time and memory usage. 

